The design, construction and performance of the MICE target

The pion-production target that serves the MICE Muon Beam consists of a titanium cylinder that is dipped into the halo of the ISIS proton beam. The design and construction of the MICE target system are described along with the quality-assurance procedures, electromagnetic drive and control systems, the readout electronics, and the data-acquisition system. The performance of the target is presented together with the particle rates delivered to the MICE Muon Beam. Finally, the beam loss in ISIS generated by the operation of the target is evaluated as a function of the particle rate, and the operating parameters of the target are derived.

==> 05-OpticalPosition/PJS-OpticalPosition.tex <==
\section{Optical Position Measurement System}
\label{Sect:OpticalPosition}

{\bf Lead authors:} Paul Smith, Chris Booth

To ensure that the trajectory of the target could be accurately controlled it
was necessary to develop a position monitoring system that would provide
continuous accurate positional information on the location of the target shaft
relative to the stator body.

As previously described the position of the shaft is tightly constrained by the
bearings and therefore its motion is one dimensional along the axis of the
stator.  Motion along a single axis can be easily monitored using a quadrature
system providing that a suitable interface can be designed.
After determining that no commercial solution was available a non-contact optical
quadrature system was designed for the target mechanism so that the controller
could continuously monitor the position of the target shaft with respect to the
stator body.

% A quadrature system is a method that is used extensively in many applications
% where either linear or rotary motion requires monitoring as it often provides
% a reliable way of ascertaining positional information for a relatively small
% footprint in terms of space and mechanical complexity. For this reason a
% quadrature system was considered a good way of obtaining the positional
% information for the target shaft.

\subsection{Description of a Quadrature System.}

A quadrature encoder is a device that converts either linear or rotary movement
into an electrical pulsed signal. A quadrature system is usually composed from
a total of three transducers and an electronic counter that work together to
give both the direction of motion and the absolute position of the moving
components.

In such a system two of these transducers ascertain both the relative movement
and the direction of movement of the system. In this document these two
transducers are referred to as channel A (CHA) and Channel B (CHB). A third
transducer is then often used to give a zero reference point or an index marker
and in this document this channel is called the index channel.
All three of these channels give a digital output so each channel can be in one
of two states at a given instance; high or low.  The distance that the system
has to move for a change of state to be observed on either of the transducers
CHA or CHB defines the resolution of the system.

CHA and CHB are arranged so that there is a phase difference between the outputs
of 90\degrees\!\!. Motion of the system under measurement in one
direction will give an output signal where the output of CHA will
lead CHB; motion in the other direction will give an output where
the output of CHB will lead CHA. The two outputs from these channels
can be interpreted as a two bit gray code giving four discrete
states. Each change of state represents a given measurable movement
of the system.  The direction in which these states change gives the
direction of motion. By counting these state changes, taking care to account
for the direction, this gives the total distance travelled by the
system.

% Figure \ref{Quadrature1} shows how this works
% diagrammatically.

The third channel, the index marker, acts a reference point that can
reset the counter. If the reset point is at a known location on the
system then multiplying the count by the resolution of the
quadrature system gives the total distance moved. The index also
acts to remove erroneous counts that could otherwise build up and
create an offset error.

% \begin{figure}[!htb]
% \begin{center}
% \scalebox{0.48}{\includegraphics {Quadrature2.png}} \caption{How a
% quadrature system can be utilised to determine position. The top
% figure illustrates how the quadrature system responds to movement in
% the positive direction. The middle figure shows how the system
% responds to movement in the negative direction. The bottom figure
% shows how the quadrature system can be utilised to keep track of the
% position when the direction of motion changes.} \label{Quadrature1}
% \end{center}
% \end{figure}

Any quadrature encoder requires an electronic interface at some
point in the system to convert the signals produced from the
quadrature transducers to digital signals for summation in an
electronic counter.  Due to the possiblity of high levels of radiation
at the location of the actuator \cite{Howlett:2007} it was recognised that
any electronics placed at this location could prematurely
fail due to radiation damage. Because of this risk it was determined
that any electronics that were part of the quadrature system needed to be well
separated from the actual sensing mechanism. Additionally the sensing mechanism
itself needed to be radiation hard and capable of reliably transmitting the
quadrature signals to the external electronics without any long term degradation
of the signal.

% Noise could
% be a problem as any errors in the positional information could lead
% to the control of the target being lost.

Some time was spent exploring the possibility of using a commercially available
quadrature encoder that could be adapted to measure the position of the target
shaft. Unfortunately there was no commercially available solution that fulfilled
the necessary requirements of having a non-contact radiation hard sensor with
the option of separating the electronics from the sensor by a signficant
distance. The result of this was that an optical quadrature system had to be
developed specifically for the target mechanism.

\subsection[Overview of the Quadrature System]{An Overview of the Quadrature Optical Position Measuring System}

To remove the necessity of having any electronics in close proximity to the target
mechanism and to ensure that the sensor was of non-contact design an optical
quadrature system was developed for the target mechanism.
Three laser sources had their light transported to the target mechanism head,
the optics block,
via single mode optical fibres. Once the fibres have entered the optics block
they are terminated onto collimators that are followed by lenses. This way the
laser light is then focused onto a graticule that is attached to the target shaft.
This graticule has many slits etched into one side of it,
each slit measuring 300\microns wide with a 300\microns spacing between each slit,
effectively creating a comb.
There a single slit etched into the other side also 300\microns wide.

Two of the channels, Channel A and Channel B, are focused onto the
comb side of the graticule whilst the Index Channel is focused onto the
side of the graticule with the single slit. The focussing is tight; the
spot size of the laser light is smaller than the half pitch of the
teeth on the graticule. This means that a single tooth, when suitably
positioned, can completely prevent the light from a given channel from passing
through to the receiving collimator. As the target shaft moves
vertically up and down inside the stator the graticule moves with the
shaft. Consequently the focused points of laser light are
alternately blocked and passed through the comb. Channel A and
Channel B are focussed so the relative positions of their focal
points are 90\degrees out of phase with respect to the teeth on the
graticule. This phase shift in the relative position of these two
collimators results in a {\lq}optical' quadrature output where the
quadrature signal can be interpreted from whether light is being
passed (or not) through the graticule on these two channels. The single
finger on the index channel is positioned two-thirds of the way down
the graticule and this gives an absolute position reference.
With slits that are 300\microns wide the quadrature system gives a positional
resolution of 150\microns\!\!.

A cartoon of the optical position measuring system designed for the target
mechanism is shown in figure \ref{OptCart}.


%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.6}{\includegraphics {OpticalCartoon1.png}} \caption{A
%cartoon illustrating the key components to the optical quadrature
%system used to ascertain the position of the target shaft.}
%\label{OptCart}
%\end{center}
%\end{figure}


The light that is passed by the vane is picked up by a separate lens
and collimator for each channel and is then transported down multi-mode
optical cables to three individual optical sensors. The optical
sensors convert the light into small electrical signals which are
then amplified and conditioned to produce the three quadrature
outputs that are required for passing into a digital counter. The
counter use to be a separate integrated circuit that was specifically
designed for counting quadrature signals. More recently the quadrature counter
has been coded into an FPGA.

\subsection{Theory}

For this system to work the spot size at the focal point must be
smaller than the pitch of the graticule. Ideally, to obtain a nice
clean signal, the focal point should be less than half the pitch of
the graticule. This then allows for a clean pass/no pass signal to
be detected as the graticule moves through the plane of the focal
point.  For the current system this entails having a focal point
that is $<$150~\microns in diameter. Ideally a focal point of less
than this is preferred as this improves the robustness of the system with
respect to slight rotational and lateral movement of the graticule in and out
of the focal plane due to the tolerances in manufacture and wear of the target
bearings.

%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.4}{\includegraphics {OpticalFocus1.png} }
%\end{center}
%\caption{Diagram showing how the collimator and lens system works
%magnifying the optical fibre source to create a finite spot size on
%the optical vane.}\label{fig:FOCALcollimator}
%\end{figure}

The simplest optical way to achieve a focal point is to focus a
parallel beam of light using a convex lens.  The collimator creates
a parallel beam from a diverging point source of light, this source
being the end of the optical fibre that is attached to the
collimator. The focusing lens and the collimator effectively work
together as a two lens system as illustrated in figure
\ref{fig:FOCALcollimator}. This optical setup will magnify the
source point by a factor of:

\begin{displaymath}
b=\frac{v}{u}a
\end{displaymath}

where \emph{b} is the image size, \emph{a} is the object size,
\emph{u} is the object focal length and \emph{v} is the image focal
length.

The object focal length is set by the collimator and for the
collimators that are used their focal length is 15.3~mm.
The image focal length is determined by physical constraints as
there is a limit as to how close to the graticule these components
can be placed. The graticule must be inside the ISIS vacuum and the
collimators and lenses must be out of the vacuum on the other side
of an optical window that separates them.  A focal distance of 45~mm is
required to acheive this. Using these figures gives a magnification factor of
three  and so the object source must be smaller than 100~\microns in diameter to
satisfy the criteria of having an image size $<$300~\microns\!\!.

Creating an object source with a diameter of less than 100~${\mu}m$
diameter whilst still having sufficient light intensity to allow a
detectable signal to pass through the system would be difficult to
achieve with a conventional light source. The use of a laser coupled
to a single mode fibre solves this problem as the end of the fibre
then acts as a very small intense source of light. As collimators are readily
available to attach directly to single mode fibres this allowed the
optical system to be constructed as described earlier.

% A measurement on the achieved spot size at the focal point on the
% vane using an early prototype with 36~mm focal length lenses showed it to have
% a FWHM of
% $\approx$75~\microns\!\!. This translates to the source of light at
% the end of the fibre being less than $\approx$25~\microns diameter.

\subsection{Details of the Optical Design}

The use of optical fibres confers an enormous advantage to this
position measurement system. The very low attenuation of the light
transmitted within the fibres allows a significant distance to be
placed between the source, receiving electronics and the optics
block. In fact, this is utilised to keep the source and the
electronics out of the synchrotron altogether.  This mitigates any
concerns about radiation damage to the electronic components and keeps the
electronics accessible at all times. In fact, both the laser source and the
receiving electronics can be kept in the MICE local control room
along with the target control electronics, a distance of 100~m away
from the target mechanism itself.

\subsection{Laser Source}

In order to assist the setting up and calibration of the optical
system a visible laser was chosen. This also has the added safety
implication that it is easy to see when the beam is on. Laser
sources at 635~nm wavelength with a controlled output power from 0
to 2.5~mW were purchased. A relatively high light output is required
because the optical losses in the system are quite high; there are a
significant number of optical interfaces, including fibre to fibre
connectors, and each interface loses light. Another reason for
maximising the light intensity through the system was because the
photodiodes that convert the light to an electrical signal do not
generate a large output voltage, typically it is of the order of a
few mV at best. Maximising the light on the sensor maximises the
devices output voltage, this in turn reduces the signal to noise
ratio and reduces the amount of amplification needed;
this significantly eases the design of the electronics.
The losses in the fibre have never been quantified, however sufficient light is
transmitted through the system that there has never been any problem obtaining
a suitable quadrature signal, even on a round trip of $\approx$200~m. Typically
the light output from the lasers is set to about 1~mW.

%This setup leaves
%overhead in both the laser light-source and the electronics in case any future
%adjustments need to be made. This facility could be important as it expected
%that the fibres close to the the synchrotron could suffer some radiation damage
%over time attenuating the light signal.

\subsection{Optical Fibres}

Two types of optical fibre were used in the system. On the
transmitting side single mode fibres were used as they give the
required small spot size at the collimator focal point ensuring a small spot
size at the vane as was illustrated earlier.
On the receiving side 200~\microns multimode fibres were used.

The single mode fibres that were used are SM600 with FC/FC
connectors.  The SM600 fibre is constructed from NuFern 630~nm fibre
\cite{NUFERN:data1} and has a pure silica core.  Silica is
considered a radiation hard material and so these fibres are ideal
for the location into which they will be going. Unfortunately no
information is available on the proton/neutron dose that these
fibres can withstand before the the fibres suffer attenuation losses
due to radiation damage.

%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.35}{\includegraphics {SM600Fibre1.png} }
%\end{center}
%\caption{The attenuation of the SM600 single mode fibre as a
%function of frequency \cite{NUFERN:data1}.}\label{fig:SM600a}
%\end{figure}

If single mode fibres were to be used on the receiving side the
collimators would have had to be aligned to a much higher precision
as the tolerance on alignment increases with a decreasing fibre
size.  Using single mode fibres could have made a system that was
difficult to set up and that could have easily gone out of
alignment. Multi-mode fibres make the alignment process much easier,
although it is still a time consuming process. 200~\micron fibres
were chosen because these minimised the cost per metre of fibre
whilst still allowing good light collection and making it relatively
easy to align the system.

The multimode fibres that are used are BFH37/200 with SMA to SMA
connectors.  These too are constructed from a 200~\microns silica
core with a fluorine silica cladding. Like the single mode fibers
the silica construction helps to ensure that the fibres have a higher
tolerance to radiation damage. Figures \ref{fig:BFH1} and
\ref{fig:BFH2} show the construction of the fibre and the
attenuation as a function of wavelength respectively
\cite{THORLAB:data1}. It can be seen from the latter that the fibre
is particulary suited to operation at 635~nm.

The fibres that were originally laid to the target in the synchrotron in
2007~??? have not shown any noticable degradation in their transmission
properties since installation. The total integrated
dose that these fibres have received since installation is unknown.

%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.4}{\includegraphics {BFH37200cross.png} }
%\end{center}
%\caption{The construction of the multimode fibre. The silica core
%gives more radiation resistance than polymer cored fibres
%\cite{THORLAB:data1}.}\label{fig:BFH1}
%\end{figure}
%
%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.4}{\includegraphics {BFH37200spectrum.png} }
%\end{center}
%\caption{ The attenuation of the BFH37/200 fibre as a function of
%frequency \cite{THORLAB:data1}.}\label{fig:BFH2}
%\end{figure}

\subsection{Collimators and Lenses}

The transmitting collimators use an FC/FC connector and
the collecting collimators use SMA connectors as this eases
identification.  The ability to connect these collimators directly
to optical fibres and their compactness has significantly simplified
the design of the system.  A collimator with a focal length of 15.3~mm
was chosen for this application; collimators with shorter focal
lengths are available.  The longer focal length minimises the
magnification of the focal spot reducing the final spot size. The
trade-off for this is that they do decrease the numerical aperture
of the collimator, theoretically making alignment a little harder.
Experience has shown that this has not proven to be a problem with
the current mounting system.

The focusing lenses are attached to the front of the collimators by
inserting the lens into a lens holder which is then screwed onto the
front of the collimator. On the transmitting side aspheric double
achromatic lenses are used to obtain the minimum spot size. On the
collecting side, where the focusing is less critical, double convex
lenses are used to re-collimate the beam.  The lenses are
$\rm{MgF_2}$ coated to minimise reflections and maximise the
light transmitted into the fibres.


\subsection{Mechanical Mount - The Optics Block}

Although the optical system was good in theory the constraints both
in terms of the physical space required to implement the system and
the requirements for a system that sat outside of the ISIS vacuum
meant that the mechanical mounting system, the optics block, went
through a significant evolution from the first prototype to the
final system that is in use today.

The construction of the optics block is all metal, with the exception of a pair
of flat sapphire windows that replaced the curved glass tube of the stator.
These windows are  bonded into a metal flange and are typical of those used for
observation in UHV environments and are rated for such use.

Each pair of collimators for each channel is held in an arm that
wraps around the mount. The{\lq}Index' and {\lq}Channel A' arms are adjustable
in the vertical direction. This allows some freedom as to where the index is set
and allows the quadrature phase to be obtained. Originally the new mount was
designed so that the collimators just slotted into the arms, however a small
modification had to be made with the addition of some small grub screws to
permit accurate alignment.

%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.5}{\includegraphics {OpticalMount2.png} }
%\end{center}
%\caption{An exploded view of the optical mount. The optical vane
%sits inside the main body where the collimators and lens caps are
%able to focus the laser light onto the vane.
%}\label{fig:OptExploded}
%\end{figure}

This mount has proven to be easy to set up and extremely robust.
Once aligned the mount proven to remain in alignment indefinitely,
even after a reasonable amount of handling. The all metal
construction of the body means that it can be sealed to the upper
flange on the stator body using a standard copper gasket, ensuring
reliable UHV operation.

%\begin{figure}[!htb]
%\begin{center}
%\scalebox{0.3}{\includegraphics {LaserOptical.jpg} }
%\end{center}
%\caption{A photo showing the laser focused onto the optical vane
%through one of the sapphire windows. It is clear from this diagram
%how small the spot size is. (The distance between fingers on the
%comb is 300~\microns\!\!.) }\label{fig:LaserVane}
%\end{figure}

\subsection{Optical Sensors}

The multimode fibres are returned to a SMA photodiode (H3R880IR).
This is a broad spectrum photodiode (400~nm to 1100~nm)
\cite{datasheet:880IR}. Given that the maximum velocity of the
target is no more than 10~ms${}^{-1}$ then this gives a maximum data
rate per channel of 33~kHz, well within the response capability of
these devices. The output from the photodiode is amplified and
conditioned before it is converted into a digital signal.

\subsection{Conclusion}

The final system has performed very well and mechanically it is
remarkably robust. Once the optical system has been aligned and
calibrated it has worked for several years without
requiring any attention.

The small amount of mechanical rotation of the target shaft that is
inevitable due to the tolerances of the components moves the
graticule into and out of the plane of focus of the laser system.
This has the effect of slightly changing the mark/space ratio of the
quadrature signals. Although the effect has been noted no problem
with counting errors has yet been observed with a correctly set up
system.



==> styles/TargetPaper_def.tex <==
%------------------------------------------------------------------------------
% New command definitions, constants, etc. for the Physics Group contribution
%                               to the ISS report
% ===========================================================================
%
%  History:
%    KL: 07Feb06: First version
%    KL: 21Aug06: Remove \eq (commented)
%    KL: 10Sep06: Add \GeV, \eV
%    KL: 05Jun07: Hyphenation options added.
%------------------------------------------------------------------------------
%	Some special symbols etc.:
%       --------------------------
%       -> small numbers
%------------------------------------------------------------------------------
\def\zero{{\scriptscriptstyle 0}}
\def\sone{{\scriptscriptstyle 1}}
\def\stwo{{\scriptscriptstyle 2}}
\def\sthr{{\scriptscriptstyle 3}}
\def\sfou{{\scriptscriptstyle 4}}
\def\sfiv{{\scriptscriptstyle 5}}
\def\sfiv{{\scriptscriptstyle 5}}
\def\ssix{{\scriptscriptstyle 6}}
\def\ssev{{\scriptscriptstyle 7}}
\def\seig{{\scriptscriptstyle 8}}
\def\snin{{\scriptscriptstyle 9}}
\def\sten{{\scriptscriptstyle 10}}
\def\half{{\scriptscriptstyle 1/2}}
%------------------------------------------------------------------------------
%       -> eV and multiples
%------------------------------------------------------------------------------
\def\Ev{\ensuremath{\text{e}\text{V\/}}}
\def\eV{\ensuremath{\text{e}\text{V\/}}}
\def\Kev{\ensuremath{\text{ke}\text{V\/}}}
\def\Mev{\ensuremath{\text{Me}\text{V\/}}}
\def\Gev{\ensuremath{\text{Ge}\text{V\/}}}
\def\GeV{\ensuremath{\text{Ge}\text{V\/}}}
\def\Gevc{\ensuremath{\text{Ge}\text{V\/}/c}}
\def\Gevcs{\ensuremath{\text{Ge}\text{V\/}/c^2}}
\def\Tev{\ensuremath{\text{Te}\text{V\/}}}
\def\ev{\ensuremath{\,\text{e}\text{V\/}}}
\def\kev{\ensuremath{\,\text{ke}\text{V\/}}}
\def\mev{\ensuremath{\,\text{Me}\text{V\/}}}
\def\gev{\ensuremath{\,\text{Ge}\text{V\/}}}
\def\gevc{\ensuremath{\,\text{Ge}\text{V\/}/c}}
\def\gevcs{\ensuremath{\,\text{Ge}\text{V\/}/c^2}}
\def\tev{\ensuremath{\,\text{Te}\text{V\/}}}
%------------------------------------------------------------------------------
%       -> various other units (for math mode only)
%------------------------------------------------------------------------------
\def\pb{\,\text{pb}}
\def\fb{\,\text{fb}}
\def\pbi{\,\text{pb}^{-1}}
\def\m{\,\text{m}}
\def\cm{\,\text{cm}}
\def\mm{\,\text{mm}}
\def\km{\,\text{km}}
\def\mum{\,\mu\text{m}}
\def\mA{\,\text{mA}}
\def\Hz{\,\text{Hz}}
\def\kHz{\,\text{kHz}}
\def\MHz{\,\text{MHz}}
\def\ppm{\,\text{ppm}}
\def\scnd{\,\text{s}}
\def\musec{\,\mu\text{s}}
\def\ns{\,\text{ns}}
\def\rad{\,\text{rad}}
\def\mrad{\,\text{mrad}}
\def\murad{\,\mu\text{rad}}
%------------------------------------------------------------------------------
%       -> commonly used symbols
%------------------------------------------------------------------------------
\def\BR{{\rm BR}}
\def\CC{{\scriptscriptstyle{\rm CC}}}
\def\CI{{\scriptscriptstyle{\rm CI}}}
\def\DA{{\scriptscriptstyle{\rm DA}}}
\def\DO{{D{\O}}\xspace}
\def\DCA{{\rm DCA}}
\def\F{{\cal F}}
\def\GRV{{\scriptscriptstyle{\rm GRV}}}
\def\IC{{\scriptscriptstyle{\rm IC}}}
\def\ISR{{\scriptscriptstyle{\rm ISR}}}
\def\IP{{\rm I$@,$P}}
\def\JB{{\scriptscriptstyle{\rm JB}}}
\def\L{{\scriptscriptstyle{\rm L}}}
\def\LL{{\scriptscriptstyle{\rm LL}}}
\def\LQbar{\overline{\rm LQ}}
\def\LQsub{{\scriptscriptstyle{\rm LQ}}}
\def\LQ{{\rm LQ}}
\def\LR{{\scriptscriptstyle{\rm LR}}}
\def\Ldes{{\cal L}_{\rm des}}
\def\Lumi{{\cal L}}
\def\MC{{\scriptscriptstyle{\rm MC}}}
\def\MSbar{\hbox{$\overline{\rm MS}$}}
\def\NC{{\scriptscriptstyle{\rm NC}}}
\def\NS{{\scriptscriptstyle{\rm NS}}}
\def\Prob{{\cal P}}
\def\QPM{{\scriptscriptstyle{\rm QPM}}}
\def\RL{{\scriptscriptstyle{\rm RL}}}
\def\RPv{{{\not R}_P}}
\def\RR{{\scriptscriptstyle{\rm RR}}}
\def\R{{\scriptscriptstyle{\rm R}}}
\def\SM{{\scriptscriptstyle{\rm SM}}}
\def\SU2U1{{\rm SU}(2)\times{\rm U}(1)}
\def\Ssup{{\scriptscriptstyle{\rm S}}}
\def\XXX{\hbox{\bf ??}}
\def\alsmu#1{{\alpha_s(\mu_{#1}^2)}}
\def\alsmz{{\alpha_s(M_Z^2)}}
\def\alsqs{{\alpha_s(Q^2)}}
\def\als{{\alpha_s}}
\def\ctwb{\cos\theta_{\scriptscriptstyle W}}
\def\ctws{\cos^2\theta_{\scriptscriptstyle W}}
\def\cut{{\rm cut}}
\def\data{{\rm data}}
\def\det{{\rm det}}
\def\dof{{\rm dof}}
\def\elm{{\rm elm}}
\def\epslam{{\epsilon/\Lambda^2}}
\def\exc{{\rm exc}}
\def\exp{{\rm exp}}
\def\gh{{\gamma_h}}
\def\had{{\rm had}}
\def\kg{{k_\gamma}}
\def\lsq#1{{\lambda_{#1}}}
\def\lsqp#1{{\lambda'_{#1}}}
\def\lsqpp#1{{{\lambda''}_{#1}}}
\def\max{{\rm max}}
\def\meas{{\rm meas}}
\def\min{{\rm min}}
\def\obs{{\rm obs}}
\def\ord#1{{\cal O}(#1)}
\def\rnge{{\,\text{--}\,}}
\def\sca{{\rm sca}}
\def\sihat{{\hat\sigma}}
\def\slim{{\rm lim}}
\def\slimb{{\rm lim,B}}
\def\slimr{{\rm lim,R}}
\def\smin{{\rm min}}
\def\smax{{\rm max}}
\def\stwb{\sin\theta_{\scriptscriptstyle W}}
\def\stwss{\sin^4\theta_{\scriptscriptstyle W}}
\def\stws{\sin^2\theta_{\scriptscriptstyle W}}
\def\sys{{\rm sys}}
\def\ta{{\theta^\ast}}
\def\tilR{\tilde R}
\def\tilS{\tilde S}
\def\tilU{\tilde U}
\def\tilV{\tilde V}
\def\tl{{\theta_\ell}}
\def\tot{{\rm tot}}
\def\true{{\rm true}}
\def\tw{\theta_{\scriptscriptstyle W}}
%------------------------------------------------------------------------------
%       -> some math symbols (+,-,...) for usage as mathchar's
%------------------------------------------------------------------------------
\mathchardef\qsm=63
\mathchardef\pls=43
\mathchardef\mns=512
\mathchardef\plm=518
\mathchardef\eql=61
\mathchardef\smallleft=300
\mathchardef\smallright=301
\mathchardef\perslsh=47
\mathchardef\les=316
\mathchardef\gre=318
\mathchardef\leq=532
\mathchardef\grq=533
%------------------------------------------------------------------------------
%       -> characters for typewriter font (used for http addresses)
%------------------------------------------------------------------------------
\chardef\usc=95
\chardef\til=126
%------------------------------------------------------------------------------
%       -> shorthand for "integral limits below and above"
%------------------------------------------------------------------------------
\def\intl{\int\limits}
%------------------------------------------------------------------------------
%       -> footenote markers
%------------------------------------------------------------------------------
\def\fdag{$^{{\displaystyle\dagger})}$}
\def\fddag{$^{{\displaystyle\ddagger})}$}
\def\fstar{$^{{\displaystyle\star})}$}
\def\faste{$^{{\displaystyle\ast})}$}
%------------------------------------------------------------------------------
%       -> d'Alembert operator
%------------------------------------------------------------------------------
\def\sqr#1#2#3{{\vcenter{\hrule height.#3ex\hbox{\vrule width.#2ex height#1ex
    \kern#1ex\vrule width.#3ex}\hrule height.#2ex}}}
\def\dalem{\mathchoice\sqr{1.6}{08}{24}\sqr{1.6}{08}{24}
                      \sqr{1.4}{07}{21}\sqr{1.1}{06}{18}}
%------------------------------------------------------------------------------
%       -> rectangle with arrow ( '-> )
%------------------------------------------------------------------------------
\def\angleto{\vrule width.035em height2.1ex depth-.56ex\unskip\kern-.6ex\to}
%------------------------------------------------------------------------------
%       -> permille sign
%------------------------------------------------------------------------------
\def\perchc#1{{\raise.4ex\hbox{$\mkern4mu#1{\it\perslsh}_
             {\mkern-5mu\scriptscriptstyle{{\rm o}\!{\rm o}}}^
             {\mkern-12.8mu\scriptscriptstyle{\rm o}}$}}}
\def\permil{{\mathchoice\perchc{\displaystyle}\perchc{\textstyle}
             \perchc{\scriptstyle}\perchc{\scriptscriptstyle}}}
%------------------------------------------------------------------------------
%       -> wide bar and bar in parantheses as mathaccents, some applications
%------------------------------------------------------------------------------
\def\widebar#1{\mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.mu}\mkern1.mu}
\catcode`\@=11 % @ signs are now treated as letters
\def\parenbar{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}
\catcode`\@=12 % @ signs are no longer letters
\def\nuan{\ensuremath{\parenbar{\nu}}}
\def\qqbar{\ensuremath{\parenbar{q}}}
\def\pbar{\ensuremath{\widebar{p}}}
\def\qbar{\ensuremath{\widebar{q}}}
\def\dbar{\ensuremath{\widebar{d}}}
\def\ubar{\ensuremath{\widebar{u}}}
\def\sbar{\ensuremath{\widebar{s}}}
\def\cbar{\ensuremath{\widebar{c}}}
\def\bbar{\ensuremath{\widebar{b}}}
\def\tbar{\ensuremath{\widebar{t}}}
\def\nubar{\ensuremath{\widebar{\nu}}}
\def\Dbar{\ensuremath{\widebar{D}}}
\def\ebar{\ensuremath{\widebar{e}}}
%------------------------------------------------------------------------------
%	Some shorthands and utilities:
%       ------------------------------
%       -> vertical rule of width zero and variable height & depth
%------------------------------------------------------------------------------
\newbox\struttbox
\setbox\struttbox=\hbox{\vrule height1.65ex depth.485ex width0pt}
\def\strutt{\relax\ifmmode\copy\struttbox\else\unhcopy\struttbox\fi}
\def\stru#1#2{\relax\ifmmode\hbox{\vrule height#1 depth#2 width0pt}
\else\vrule height#1 depth#2 width0pt\fi}
%------------------------------------------------------------------------------
%       -> underline with resonable distance text - line
%------------------------------------------------------------------------------
\def\uline#1{$\underline{\hbox{#1\strutt}}$}
%------------------------------------------------------------------------------
%       -> roman numbers (uppercase and lowercase)
%------------------------------------------------------------------------------
\def\ronum#1{\uppercase\expandafter{\romannumeral#1}}
\def\ronuml#1{\expandafter{\romannumeral#1}}
%------------------------------------------------------------------------------
%       -> vectors and matrices
%------------------------------------------------------------------------------
\def\vect#1{\begin{matrix}#1\end{matrix}}
\def\pvect#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bvect#1{\begin{bmatrix}#1\end{bmatrix}}
%------------------------------------------------------------------------------
%       -> some alignment tools for tables
%------------------------------------------------------------------------------
\def\cA{{\phantom{0}}}
\def\cB{{\phantom{00}}}
\def\cC{{\phantom{000}}}
\def\cD{{\phantom{0000}}}
\def\cM{{\phantom{\mns}}}
%------------------------------------------------------------------------------
%       -> shorthand for protected citations in captions
%------------------------------------------------------------------------------
\def\pcite#1{\protect\cite{#1}}
%------------------------------------------------------------------------------
%       -> shorthands for equation, figure, table, section references
%------------------------------------------------------------------------------
%\def\eq#1{eq.~(\ref{eq-#1})}
\def\eqsand#1#2{eqs.~(\ref{eq-#1}) and~(\ref{eq-#2})}
\def\eqsto#1#2{eqs.~(\ref{eq-#1}-\ref{eq-#2})}
\def\eqstwo#1#2{eqs.~(\ref{eq-#1},\ref{eq-#2})}
\def\eqsthr#1#2#3{eqs.~(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3})}
\def\eqsfou#1#2#3#4{eqs.~(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3},\ref{eq-#4})}
\def\Eq#1{Equation~(\ref{eq-#1})}
\def\Eqsto#1#2{Equations~(\ref{eq-#1}-\ref{eq-#2})}
%\def\fig#1{Fig.~\ref{fig-#1}}
\def\figs#1{Fig.~\ref{fig-#1}}
\def\Fig#1{Figure~\ref{fig-#1}}
\def\figand#1#2{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\def\figand#1#2{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\def\tab#1{Table~\ref{tab-#1}}
\def\tabsand#1#2{Tables~\ref{tab-#1} and~\ref{tab-#2}}
\def\Tab#1{Table~\ref{tab-#1}}
\def\sec#1{Sect.~\ref{sec-#1}}
\def\Sec#1{Section~\ref{sec-#1}}
\def\secand#1#2{Sects.~\ref{sec-#1} and~\ref{sec-#2}}
\def\secsto#1#2{Sects.\ref{sec-#1} to~\ref{sec-#2}}
%------------------------------------------------------------------------------
%	Local laguage changes
%       ---------------------
%------------------------------------------------------------------------------
\def\german#1{\selectlanguage{german}#1\selectlanguage{english}}
%------------------------------------------------------------------------------
%	Redefine mathbf
%       ---------------
%------------------------------------------------------------------------------
%\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{sl}
\def\mb{\mathbf}
%------------------------------------------------------------------------------
%
% New commands:
%
%------------------------------------------------------------------------------
%
\newcommand{\address}{ } 
%
\newcommand{\gevsq}     {\mbox{${\rm GeV}^2$}}
\newcommand{\qsd}       {\mbox{${Q^2}$}}
\newcommand{\PTM}       {P_{T\rm miss}}
\newcommand{\x}         {\mbox{${\it x}$}}
\newcommand{\y}         {\mbox{${\it y}$}}
\newcommand{\ye}        {\mbox{${y_{e}}$}}
\newcommand{\smallqsd}  {\mbox{${q^2}$}}
\newcommand{\rambox}    {\mbox{$ \rightarrow $}}
\newcommand{\ra}        {$\rightarrow$}
\newcommand{\ygen}      {\mbox{${y_{gen}}$}}
\newcommand{\yjb}       {\mbox{${y_{_{JB}}}$}}
\newcommand{\yda}       {\mbox{${y_{_{DA}}}$}}
\newcommand{\qda}       {\mbox{${Q^2_{_{DA}}}$}}
\newcommand{\qjb}       {\mbox{${Q^2_{_{JB}}}$}}
\newcommand{\ypt}       {\mbox{${y_{_{PT}}}$}}
\newcommand{\qpt}       {\mbox{${Q^2_{_{PT}}}$}}
\newcommand{\ypr}       {\mbox{${y_{(1)}}$}}
\newcommand{\yprpr}     {\mbox{${y_{(2)}}$}}
\newcommand{\ypps}      {\mbox{${y_{(2)}^2}$}}
\newcommand{\gammah}    {\mbox{$\gamma_{_{H}}$}}
\newcommand{\gammahc}   {\mbox{$\gamma_{_{PT}}$}}
\newcommand{\gap}       {\hspace{0.5cm}}
\newcommand{\gsim}      {\mbox{\raisebox{-0.4ex}{$\;\stackrel{>}{\scriptstyle \sim}\;$}}}
\newcommand{\lsim}      {\mbox{\raisebox{-0.4ex}{$\;\stackrel{<}{\scriptstyle \sim}\;$}}}
\renewcommand{\thefootnote}{\arabic{footnote}}
%
%----------------------------------------------------------------------------
%
% Constants etc.
% ==============
%
%----------------------------------------------------------------------------
% Define (e.g.) working value of theta_23?
%
%----------------------------------------------------------------------------
%
% Paper format
% ============
%
%----------------------------------------------------------------------------
%
%------------------------------------------------------------------------------
%	page layout
%------------------------------------------------------------------------------
\paperheight    29.7cm
\paperwidth     21.0cm
%------------------------------------------------------------------------------
%	... horizontal spacings
%------------------------------------------------------------------------------
\textwidth      16.0cm
\evensidemargin -0.3cm
\oddsidemargin  -0.3cm
%------------------------------------------------------------------------------
%	... vertical spacings
%------------------------------------------------------------------------------
\textheight     650.pt
%\topmargin      -1.5cm -- KL 18Apr06
\footskip        1.0cm
%------------------------------------------------------------------------------
%	interline spacing, paragraph indention etc.
%------------------------------------------------------------------------------
\renewcommand{\baselinestretch}{1.12}
\renewcommand{\arraystretch}{1.1}
\parindent       0.0pt
\parskip         0.3cm plus0.05cm minus0.05cm
\overfullrule    0.0pt
%------------------------------------------------------------------------------
%	item spacings
%------------------------------------------------------------------------------
\itemsep    0.2ex plus 0.1ex minus 0.15ex
\topsep     0.2ex plus 0.1ex minus 0.15ex
\partopsep  1.2ex plus 0.6ex minus 0.6ex
\setlength\leftmargini   {1.6em}
\setlength\leftmarginii  {1.4em}
\setlength\leftmarginiii {1.2em}
\setlength\leftmarginiv  {1.0em}
%------------------------------------------------------------------------------
%	"tight item" environments
%------------------------------------------------------------------------------
\newenvironment{tightitemize}[2]
 {\begin{list}{$\bullet$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
\newenvironment{tightsubitemize}[2]
 {\begin{list}{$-$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
\newenvironment{tightssubitemize}[2]
 {\begin{list}{$\to$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
%------------------------------------------------------------------------------
%	float parameters
%------------------------------------------------------------------------------
\renewcommand{\topfraction}{1.}
\renewcommand{\bottomfraction}{1.}
\renewcommand{\textfraction}{0.01}
\setlength{\floatsep}{6pt plus 3pt minus 3pt}
\setlength{\textfloatsep}{12pt plus 8pt minus 4pt}
%------------------------------------------------------------------------------
%	adjust footnote design
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newlength{\@fninsert}
\setlength{\@fninsert}{0.6em}
\newlength{\@fnwidth}
\setlength{\@fnwidth}{\textwidth}
\addtolength{\@fnwidth}{-\@fninsert}
\addtolength{\@fnwidth}{-0.4em}
\renewcommand{\@makefntext}[1]%
  {\noindent\makebox[\@fninsert][r]{\@makefnmark}\hfil%
  \parbox[t]{\@fnwidth}{#1}}
\catcode`\@=12 % @ signs are no longer letters
\addtolength{\skip\footins}{2.mm}
%------------------------------------------------------------------------------
%	equation numbers like (n.k): n=section, k=equation
%------------------------------------------------------------------------------
%\numberwithin{equation}{section}
%\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
%------------------------------------------------------------------------------
%	set section numbering depth (5: allow for sections up to i.j.k.l.m.)
%       and redefine section, subsection, subsubsection, paragraph 
%       to yield a proper heading
%       force four levels of headers in the table of contents
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\setcounter{secnumdepth}{5}
\setcounter{tocdepth}{4}
\renewcommand\section{\@startsection{section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalfont\Large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-3.25ex\@plus -1ex \@minus -.2ex}%
                                   {1.5ex \@plus .2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {-3.25ex\@plus -1ex \@minus -.2ex}%
                                   {1.5ex \@plus .2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {3.25ex \@plus1ex \@minus.2ex}%
                                   {1.2ex \@plus .2ex}%
                                   {\normalfont\normalsize\bfseries}}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%	separators for subsections and sections
%------------------------------------------------------------------------------
\def\sectionsep{\strut}
\def\chaptersep{\vfill\eject}
%------------------------------------------------------------------------------
%	Add hyphenation options
%------------------------------------------------------------------------------
\hyphenation{par-ti-cu-lar} \hyphenation{ex-pe-ri-men-tal}
\hyphenation{dif-fe-rent} \hyphenation{bet-we-en}
\hyphenation{mo-du-lus}
%
%--------  End  --------  --------  --------  --------  --------  --------

